Adversarial Nibbler: A Data-Centric Challenge for Improving the Safety of Text-to-Image Models

The generative AI revolution in recent years has been spurred by an expansion in compute power and data quantity, which together enable extensive pre-training of powerful text-to-image (T2I) models. With their greater capabilities to generate realistic and creative content, these T2I models like DALL-E, MidJourney, Imagen or Stable Diffusion are reaching ever wider audiences. Any unsafe behaviors inherited from pretraining on uncurated internet-scraped datasets thus have the potential to cause wide-reaching harm, for example, through generated images which are violent, sexually explicit, or contain biased and derogatory stereotypes. Despite this risk of harm, we lack systematic and structured evaluation datasets to scrutinize model behavior, especially adversarial attacks that bypass existing safety filters. A typical bottleneck in safety evaluation is achieving a wide coverage of different types of challenging examples in the evaluation set, i.e., identifying 'unknown unknowns' or long-tail problems. To address this need, we introduce the Adversarial Nibbler challenge. The goal of this challenge is to crowdsource a diverse set of failure modes and reward challenge participants for successfully finding safety vulnerabilities in current state-of-the-art T2I models. Ultimately, we aim to provide greater awareness of these issues and assist developers in improving the future safety and reliability of generative AI models. Adversarial Nibbler is a data-centric challenge, part of the DataPerf challenge suite, organized and supported by Kaggle and MLCommons.

==> old_text.tex <==
%%% ABSTRACT
%Briefly describe your competition:
%summarize the background, available data, methods, available baseline, and potential impact. \textbf{The proposal should not exceed 8 pages in total (references and bios excluded)}.
% Machine learning progress has been strongly influenced by the data used for model training and evaluation. Only recently however, have development teams shifted their focus more to the data. This shift has been triggered by the numerous reports about biases and errors discovered in AI datasets. Thus, the data-centric AI movement introduced the notion of iterating on the data used in AI systems, as opposed to the traditional model-centric AI approach, which typically treats the data as a given static artifact in model development. With the recent advancement of generative AI, the role of data is even more crucial for successfully developing more factual and safe models. DataPerf challenges follow up on recent successful data-centric challenges drawing attention to the data used for training and evaluation of machine learning model. Specifically, Adversarial Nibbler focuses on data used for safety evaluation of generative text-to-image models. A typical bottleneck in safety evaluation is achieving a representative diversity and coverage of different types of examples in the evaluation set. Our competition aims to gather a wide range of long-tail and unexpected failure modes for text-to-image models in order to identify as many new problems as possible and use various automated approaches to expand the dataset to be useful for training, finetuning, and evaluation. 

% Machine learning has advanced significantly, largely due to the quantity of data used in model training and evaluation. Generative AI has made high-quality data even more crucial as they are capable of producing realistic and creative content, but they can also be used to generate harmful or misleading content since they are trained on large datasets of real-world data, which can include biases, errors, and harmful content. As a result, it is imperative to ensure that machine learning models are accurate and reliable to prevent the generation of harmful or misleading content. A typical bottleneck in safety evaluation is achieving a representative diversity and coverage of different types of examples in the evaluation set. But the challenge lies in getting access to this high-quality data. To address this need, we introduce the \textit{Adversarial Nibbler} challenge. The goal of our challenge is to construct a diverse set of insightful examples of long tail problems for text-to-image models that will help to improve the safety and reliability of generative AI models. Through the competition, we will crowdsource the diverse failure modes to identify new problems and uses automation to expand the dataset for training, fine-tuning, and evaluation. Adversarial Nibbler is a data-centric challenge that is part of the DataPerf suite, which is organized and supported by Kaggle and MLCommons.

%% INTRO/BACKGROUND
 

 %For example, a T2I model might be trained on a dataset of images that includes both positive and negative examples of a certain concept. If the model is not carefully designed, it could generate images that are harmful or offensive, even if it was not explicitly trained to do so.
% Another challenge is that T2I models can be susceptible to adversarial attacks. An attacker could intentionally feed the model a text prompt that is designed to generate a harmful or undesirable image. For example, an attacker could use a text prompt that contains hate speech or that promotes violence.


% With the advent of conversational agents such as ChatGPT and text-to-image generators such as DALL-E \citep{dalle2021,dalle2022}, Midjourney\footnote{https://docs.midjourney.com/}, Imagen \citep{imagen2022}, Stable Diffusion \citep{stable-diffusion-2021}, among many others, we are on the cusp of Generative Artificial Intelligence (GenAI) models demonstrating capabilities that will revolutionize the landscape of visual content creation and dissemination. These models require large amounts of training data and their biases/learnt representations depend intimately on what is and is not included in these training sets. Most machine learning failures with negative downstream effects occur due to issues with data being insufficient, biased or outdated, and yet data is the most under-valued and de-glamorised aspect of AI \citep{Sambasivan2021}.


%% NOVELTY
% Generative text-to-image models commonly integrate text-based filters to identify generation requests that may be overtly harmful. However, empirical studies demonstrate that such filters fall short in comprehensively safeguarding against the complete range of potential hazards. To this end, we are proposing a novel and new challenge that targets the identification and mitigation of failure modes that can circumvent extant safety filters, thereby addressing this gap in the current state of the art.

% The goal of the Adversarial Nibbler challenge is to engage the research community in jointly discovering a diverse set of insightful long tail problems for text-to-image models and thus help identify current blind spots in harmful image generation (i.e., unknown unknowns). We focus on prompt-image pairs that currently slip through the cracks of safety filters -- either via intentful \textit{subversive prompts} that circumvent the text-based filters or through seemingly \textit{benign requests} that nevertheless trigger unsafe outputs. By focusing on unsafe generations paired with seemingly safe prompts, our challenge zeros in on cases that (i) are most challenging to catch via text-prompt filtering alone and (ii) have the potential to be very harmful to non-adversarial end users. 

% This challenge is a timely response to identify and mitigate safety concerns in a structured and systematic manner, covering both the discovery of new failure modes and the confirmation of existing ones. 
% With Adversarial Nibbler we propose a way to scale the process of seeding unique and diverse adversarial examples. This competition is the result of wide collaboration between six different organizations from academia and industry to jointly produce a shared resource for use and reuse by the wider research and development community. It is one of multiple data-centric challenges launched by the DataPerf organization in collaboration with the Kaggle community.

%Participants are simply required to devise an ostensibly safe prompt (i.e., benign or subversive), and subsequently select an image displaying unsafe generation from the outputs of multiple text-to-image models. Participants are then expected to describe the unsafe generation by responding to four questions pertaining to (1) the attack used in the prompt, (2) the description of harm apparent in the image, (3) the type of harm inflicted, and (4) the identity attributes targeted in the image.
